Specification Testing for Dyadic Regression Models

Of the 88 empirical papers on dyadic or other relational data that we reviewed in the top five economics journals, 55 (62.5\%) use a linear specification. To assess whether such a specification describes the conditional mean, we develop Kolmogorov-Smirnov and Cram\'er-von Mises tests for undirected dyadic data that also accommodate smooth nonlinear specifications. To our knowledge, this paper is the first to develop omnibus specification tests for undirected dyadic regression models. A corrected first-order multiplier bootstrap is asymptotically exact in two standard Gaussian cases: the first-order nondegenerate case and independent dyads case. For a general class of such processes, we establish that a second-order multiplier bootstrap consistently approximates the limiting law uniformly over the indexing function class, even when the indexing functions are estimated. For the specification tests, we augment this bootstrap to account for two additional sources of non-Gaussianity: parameter estimation and the curvature of the regression function. We then construct an envelope test that is asymptotically exact in both Gaussian cases and controls size in the other degenerate cases. Simulations illustrate the size and power of the tests. In an application to housing sales, we reject a common mean price gap within distance bands but do not reject separate linear relationships by metro access.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
